The Impact of Background Removal on Performance of Neural Networks for Fashion Image Classification and Segmentation

Fashion understanding is a hot topic in computer vision, with many applications having great business value in the market. Fashion understanding remains a difficult challenge for computer vision due to the immense diversity of garments and various scenes and backgrounds. In this work, we try removing the background from fashion images to boost data quality and increase model performance. Having fashion images of evident persons in fully visible garments, we can utilize Salient Object Detection to achieve the background removal of fashion data to our expectations. A fashion image with the background removed is claimed as the "rembg" image, contrasting with the original one in the fashion dataset. We conducted extensive comparative experiments with these two types of images on multiple aspects of model training, including model architectures, model initialization, compatibility with other training tricks and data augmentations, and target task types. Our experiments show that background removal can effectively work for fashion data in simple and shallow networks that are not susceptible to overfitting. It can improve model accuracy by up to 5% in the classification on the FashionStyle14 dataset when training models from scratch. However, background removal does not perform well in deep neural networks due to incompatibility with other regularization techniques like batch normalization, pre-trained initialization, and data augmentations introducing randomness. The loss of background pixels invalidates many existing training tricks in the model training, adding the risk of overfitting for deep models.

==> sections/preliminaries.tex <==
In this work, we assess the impact of background removal from fashion images on the performance of networks with CNN and Transformer architectures in image classification and segmentation tasks. This section provides an overview of the related background, including methods, models, and techniques we use in this work, namely, transfer learning, CNNs and transformers, salient object detection, instance segmentation, and semantic segmentation. We also provide an overview of related work. 

\subsection{Transfer Learning.} Transfer learning~\cite{tan_survey_2018} was born for the problem of reusing model training and data dependence of deep learning. Specifically, via transfer learning, the model in the target domain is not required to be trained from scratch, and it can reuse the model parameters from another related task and make it serve as a weight initialization for the target model, which is intuitively described as transferring the knowledge from one domain to another. After the initialization of pre-trained model parameters, the model of the target domain needs to train the last layer or parts of the network to achieve convergence and better performance, usually described as the fine-tuning of models. The training and test data are not required to be identically distributed via transfer learning, which can tremendously reduce the demand for training data, making transfer learning popular and widely used in deep learning. %Deep learning models usually can reach better performance with faster training speed through transfer learning. 

In this work, we apply transfer learning as pre-trained initialization for the models, and all the pre-trained weight parameters originated from ImageNet~\cite{deng_imagenet_nodate}. It is one of the concerns of our controlled experiments.

\subsection{Convolutional Neural Networks.}
\iffalse
CNN~\cite{dumoulin_guide_2018} is a classic Artificial Neural Network (ANN) specially designed for image tasks and understanding. Nowadays, CNN is the mainstream in computer vision, commonly used for many tasks such as image classification, object detection, image segmentation, etc. The core component of CNN includes three layers: convolutional, pooling, and fully connected. The input is usually an image matrix with RGB channels. The convolutional layer is responsible for the convolutional operation, which uses learnable kernels or filters to extract the features from the images. A convolutional kernel slides spatially over the input from the previous layers. It computes dot products between the kernel and the specific region of input by stacking across the channels, finally producing a feature map for the next layer. The pooling layer is designed for down-sampling operation between successive convolutional layers, decreasing the number of model parameters and making model training feasible. With the flattened feature map as input, fully connected layers play the role of classifier in the traditional classification, aiming to predict outputs by the feature map extracted by the previous layers. 

In this work, to assess the impact of background removal in fashion images on the performance of convolutional neural networks for image classification, we have chosen the following CNNs for our experiments:  VGG11, VGG13, VGG16, VGG19~\cite{simonyan_very_2015} as the representative models of shallow and simple networks, ResNet-50~\cite{he_deep_2015}, ResNet-101~\cite{he_deep_2015} standing for typical deep neural networks, ResNeSt-101~\cite{zhang_resnest_2020} as a supplementary to the deep networks with the attention architecture. To evaluate the impact of background removal in the image instance segmentation task with CNNs, we used ResNeXt-101 and ResNeSt-101.
\fi

CNN~\cite{dumoulin_guide_2018} is a widely used Artificial Neural Network for image processing and understanding. It has become the mainstream approach in computer vision, applied in various tasks such as image classification, object detection, and image segmentation. The core components of CNN are the convolutional, pooling, and fully connected layers. The convolutional layer extracts features from images using learnable kernels, while the pooling layer down-samples the feature maps, reducing model parameters and enabling efficient training. The fully connected layers serve as classifiers for output prediction based on the extracted features. 

In our study, we evaluate the impact of background removal on the performance of CNNs for image classification and segmentation. We selected VGG11, VGG13, VGG16, and VGG19~\cite{simonyan_very_2015} as representative of shallow and simple models, ResNet-50~\cite{he_deep_2015}, ResNet-101~\cite{he_deep_2015} as typical deep networks, and ResNeSt-101~\cite{zhang_resnest_2020} as a deep network with attention architecture. For image instance segmentation, we used ResNeXt-101 and ResNeSt-101 to assess the impact of background removal on the model's performance.

\subsection{Attention and Transformers}
The Transformer~\cite{vaswani_attention_2017} is a deep learning architecture model first proposed in Natural Language Processing (NLP) domain that can perform better than the previous dominant models based on complex recurrent or convolutional neural networks. The Transformer is based on attention mechanisms, replacing recurrence and convolutions entirely. It follows the classic sequence model architecture of an encoder-decoder structure, where the encoder can be separately used to extract features. The encoder comprises a stack of N identical layers, each having two sub-layers: a multi-head self-attention mechanism and a position-wise fully connected feed-forward network.

\subsection{Salient Object Detection}\label{subsec:SOD}
Salient Object Detection (SOD) has been an attractive topic in computer vision, aiming to segment visually salient object regions in images. 
%, as illustrated in Figure~\ref{fig:sample of SOD}. 
SOD is a special kind of semantic segmentation that predicts a binary mask of salient objects, a binary classification on each pixel. Note that SOD differs from object detection with bounding box detection of the image instances. Naturally, one can use a SOD method, e.g., $U^2$-Net~\cite{qin_u2-net_2020}, to remove the background of fashion images. 
In this work, for background removal on fashion data, we used the SOD tool called Rembg~\cite{gatis_rembg_2022} based on $U^2$-Net~\cite{qin_u2-net_2020}, which is a two-level nested U-structure without using any pre-trained backbones from image classification. It can achieve comparable performance even training from scratch. Besides, thanks to the novel architecture, the network can go deeper and attain high resolution without tremendously increasing computation costs. Refer to~\cite{qin_u2-net_2020} for a detailed description of the $U^2$-Net architecture. 

\iffalse
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/sample of SOD.png}
    \caption{Samples of Salient Object Detection using Rembg tool.~\cite{gatis_rembg_2022}}
    \label{fig:sample of SOD}
\end{figure}
\fi

\subsection{Image Segmentation}\label{subsec:image segmentation}
Image segmentation is critical in fashion understanding and plays a significant role in various applications. It can be formulated into three categories, classifying pixels with semantic labels (semantic segmentation), partitioning of individual objects (instance segmentation), or both (panoptic segmentation)~\cite{minaee_image_2020}. In this work, apart from fashion image classification, we conduct a comparative assessment of the impact of background removal on the performance of NN-based instance and semantic segmentation of fashion images.

Instance segmentation is to segment individual objects in the image, which means even two objects belonging to one class are still separately partitioned for two individuals. Essentially, instance segmentation enlarges the scope of semantic segmentation by detecting and delineating each region of objects in the image~\cite{minaee_image_2020}.  Mask R-CNN~\cite{he_mask_2018} is a highly influential model for instance segmentation. It efficiently detects objects in images by extending the Faster R-CNN~\cite{ren_faster_2016} framework. It incorporates three output branches: one for bounding box regression, another for class classification, and the third for generating binary masks to segment instances. The model applies a multi-task loss on each sampled Region of Interest (ROI) to combine the losses for bounding box coordinates, class classification, and segmentation masks. The backbone architecture used for feature extraction can be any existing model, while the network head for bounding box recognition and mask generation operates on each ROI proposed by RPN~\cite{ren_faster_2016}. In this work, all the instance segmentation models we considered are based on the Mask R-CNN framework with various backbone architectures. Mask R-CNN and its extensions adopt a "detect-then-segment" strategy. We do not consider other segmentation models with different strategies.

Semantic segmentation involves labeling each pixel in an image with an object category, resulting in a semantic image with categorical pixel values. Fully Convolutional Networks (FCNs)~\cite{shelhamer_fully_2016} are significant in deep learning for semantic segmentation, as they use only convolutional layers and output segmentation maps of the same size as the input image. Another popular architecture is the encoder-decoder framework~\cite{minaee_image_2020}, where the encoder extracts features and the decoder generates semantic images through deconvolution operations. U-Net~\cite{ronneberger_u-net_2015} is an excellent model based on this framework, known for efficient medical image segmentation. Various extensions of U-Net~\cite{zhou_unet_2018}, \cite{huang_unet_2020} exist for different domains. 

Since semantic segmentation annotations cover the background, background removal with SOD methods may not significantly benefit semantic segmentation. In this study, we evaluate the impact of background removal using the SOD method on fashion image semantic segmentation, specifically using Swin-B (Swin Transformer-Base)~\cite{liu_swin_2021-1}.


